Software Entity Recognition with Noise-Robust Learning

Recognizing software entities such as library names from free-form text is essential to enable many software engineering (SE) technologies, such as traceability link recovery, automated documentation, and API recommendation. While many approaches have been proposed to address this problem, they suffer from small entity vocabularies or noisy training data, hindering their ability to recognize software entities mentioned in sophisticated narratives. To address this challenge, we leverage the Wikipedia taxonomy to develop a comprehensive entity lexicon with 79K unique software entities in 12 fine-grained types, as well as a large labeled dataset of over 1.7M sentences. Then, we propose self-regularization, a noise-robust learning approach, to the training of our software entity recognition (SER) model by accounting for many dropouts. Results show that models trained with self-regularization outperform both their vanilla counterparts and state-of-the-art approaches on our Wikipedia benchmark and two Stack Overflow benchmarks. We release our models, data, and code for future research.

==> fables/fig_sentence_length_distribution.tex <==
\begin{figure}[t]
\vspace{-0.1in}
    \centering
    \includegraphics[width=1\columnwidth]{figs/sentence_length_distribution.pdf}
    \caption{Distribution of sentence lengths in \textsc{WikiSER}.
    }
    \label{fig_sentence_length_distribution}
\end{figure}


==> fables/fig_span.tex <==
\begin{figure}[t]
    \centering
    \vspace{-0.1in}
    \includegraphics[width=0.9\columnwidth]{figs/span.pdf}
    \vspace{-0.1in}
    \caption{Example of a challenging input with nested spans.}
    \label{fig_span}
\end{figure}

==> fables/tab_baselinewikispan.tex <==
\begin{table}[t]
    \caption{Accuracy of Entity Span Detection}
    \centering
    \begin{tabular}{llll}
    \toprule
        & Precision & Recall & F1 \\
        \midrule
        BERTOverflow & 75.8 & 77.6 & 76.7 \\
        BERT$_{base}$ & 77.3 & 82.1 & 79.6 \\
        BERT$_{base}$ + Self-reg. & \textbf{80.9} & \textbf{80.5} & \textbf{80.7} \\
    \bottomrule
    \end{tabular}
    \label{tab_baselinewikispan}
\end{table}

==> fables/tab_page-examples.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[t]
\caption{Software Entity Types and Examples in \textsc{WikiSER}}
\resizebox{\columnwidth}{!}{% 
\begin{tabular}{lc}
\toprule
% \multicolumn{1}{c}{Type} & Examples \\
\multicolumn{1}{c}{Type} & Examples \\
\midrule
Algorithm        & \begin{tabular}[c]{@{}c@{}} \emph{Auction algorithm, Collaborative filtering} \end{tabular}       \\
Application               & \begin{tabular}[c]{@{}c@{}}\emph{Adobe Acrobat, Microsoft Excel} \end{tabular}       \\
Architecture      & \begin{tabular}[c]{@{}c@{}}\emph{Graphics processing unit, Wishbone}
%(computer bus)
\end{tabular}
\\
Data Structure            & \begin{tabular}[c]{@{}c@{}}\emph{Array, Hash table, mXOR linked list}\end{tabular}                \\
Device                     & \begin{tabular}[c]{@{}c@{}}\emph{Samsung Gear S2, iPad, Intel T5300}\end{tabular}    \\
Error Name                & \begin{tabular}[c]{@{}c@{}}\emph{Buffer overflow, Memory leak}\end{tabular}              \\
General Concept  & \begin{tabular}[c]{@{}c@{}}\emph{Memory management %(operating systems)
, Nouvelle AI}\end{tabular}         \\
Language                   & \begin{tabular}[c]{@{}c@{}}\emph{C++, Java, Python, Rust} %(programming language)
\end{tabular}     \\
Library                    & \begin{tabular}[c]{@{}c@{}}\emph{Beautiful Soup%(HTML parser) 
, FastAPI} \end{tabular} \\
License                    & \begin{tabular}[c]{@{}c@{}}\emph{Cryptix General License, MIT License}\end{tabular} \\
Operating System & \begin{tabular}[c]{@{}c@{}}\emph{Linux, Ubuntu, Red Hat OS, MorphOS} %(real-time operating system)
\end{tabular}       \\
Protocol                   & \begin{tabular}[c]{@{}c@{}}\emph{TLS, FTPS, HTTP 404}\end{tabular} \\
\bottomrule
\end{tabular}
}
\label{tab_page-example}
\end{table}
